LoRA and Privacy: When Random Projections Help (and When They Don't)

We introduce the (Wishart) projection mechanism, a randomized map of the form $S \mapsto M f(S)$ with $M \sim W_d(1/r I_d, r)$ and study its differential privacy properties. For vector-valued queries $f$, we prove non-asymptotic DP guarantees without any additive noise, showing that Wishart randomness alone can suffice. For matrix-valued queries, however, we establish a sharp negative result: in the noise-free setting, the mechanism is not DP, and we demonstrate its vulnerability by implementing a near perfect membership inference attack (AUC $> 0.99$). We then analyze a noisy variant and prove privacy amplification due to randomness and low rank projection, in both large- and small-rank regimes, yielding stronger privacy guarantees than additive noise alone. Finally, we show that LoRA-style updates are an instance of the matrix-valued mechanism, implying that LoRA is not inherently private despite its built-in randomness, but that low-rank fine-tuning can be more private than full fine-tuning at the same noise level. Preliminary experiments suggest that tighter accounting enables lower noise and improved accuracy in practice.

==> content/experiments.tex <==
The Gaussian baseline that ignores the randomness in \(M\) corresponds to standard DP-SGD: since \(V^\top=\nabla_W \cL(W_t)\), privatizing \(V\) directly (treating \(M\) as post-processing) amounts to adding Gaussian noise to the full gradient matrix, i.e., updating without any low-rank projection.

We emphasize that our mechanism \(\cA_2\) is not identical to the standard implementation of DP-LoRA-FA. In our analysis, we add Gaussian noise to \(V^\top=\nabla_W \cL(W_t)\) and then apply the random projection. In contrast, DP-LoRA-FA adds noise after first multiplying by \(A^\top\), i.e., to \(\nabla_W \cL(W_t)A^\top\). We focus on the former variant because it admits a more tractable theoretical analysis. Nonetheless, Appendix~\ref{app:subsec-comparison-dp-lora-small-r} shows that, with high probability, the two procedures inject noise of the same order. Moreover, our implementation does not require explicitly forming the full matrix gradient \(\nabla_W \cL(W_t)\): it can be realized using only gradients with respect to the trainable LoRA factor $B$~(\Cref{algo:lora-add-noise-1}), preserving the computational motivation of LoRA. For completeness, we include the standard DP-LoRA-FA implementation in our experiments.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.97\linewidth]{fig/dp_lora_vs_ours_plots.png}
    \caption{Comparison of DP-SGD, DP-LoRA, and our noisy LoRA~(\ref{eq:M2}) with our accounting method in~\Cref{thm:matrix-dp-proj-mechanism-small-r}}
    \label{fig:comparison}
\end{figure}
For an empirical comparison of these different methods, we fine-tune on CIFAR-10 to compare our method (\ref{eq:M2} with the privacy accounting from \Cref{thm:matrix-dp-proj-mechanism-small-r}) with DP-Lora-FA and DP-SGD under the same privacy budget.
Appendix~\ref{app:subsec-comparison-exp-details} provides implementation details (backbone, hyper-parameter grid, and accounting). 

\Cref{fig:comparison} (right) reports test accuracy as a function of the privacy budget $\varepsilon$ for $\delta = 10^{-4}$. In the small $\varepsilon$ regime, our method (and DP-LoRA at extremely low $\varepsilon$) outperforms DP-SGD, since the low-rank projection reduces the amount of noise required to achieve a given privacy level. \jd{is there a regime where our method outperform dp-sgd and dp-lora doesn't? if yes we should mention that no?} As $\varepsilon$ increases, the required noise decreases for all methods and this advantage diminishes. In the large $\varepsilon$ regime the accuracy gains from reduced noise are outweighed by the optimization bias introduced by the low-rank constraint, so DP-SGD matches or slightly outperforms our approach.

In~\Cref{fig:comparison} (left), we isolate the effect of the low-rank projection by comparing our method $\cA_2$ across ranks $r$ at a fixed privacy budget. While the two approaches are similar and, with high probability, add effective noise of the same order (see Appendix~\ref{app:subsec-comparison-dp-lora-small-r} for details), we observe that our Wishart projection is consistently better, especially at smaller ranks. This suggests that beyond the amount of injected noise, the geometry of the random projection (applied to both the gradient matrix and the noise) also affects model utility. Understanding when and why different projection distributions perform better remains an interesting direction for future work.


==> content/matproj_gaussian_comp.tex <==
\subsubsection{Comparison with the Classical Gaussian Mechanism}\label{subsec:compare-classical}
\as{Have not edited below}
We next compare the privacy guarantee in \Cref{thm:matrix-large-r-main} to a classical baseline that ignores the intrinsic randomness in $M$. The baseline treats $V\mapsto MV$ as deterministic, applying the Gaussian mechanism calibrated to the Frobenius sensitivity.


\noindent\textbf{Setup.}
Fix \(V,V'\in\mathbb{R}^{d\times n}\). Let \(J=J(V,V')\) with \(k \coloneqq |J|\). Assume \(\|v_j\|_2=\|v'_j\|_2=1\) and \(\|v_j-v'_j\|_2\le \Delta_v\) for all \(j\in J\) (e.g., \Cref{eq:Deltav}), then
\begin{equation}
\label{eq:DV-frob-cmpr}
\|\Delta V\|_F^2=\sum_{j\in J}\|v_j-v'_j\|_2^2 \le k\Delta_v^2.
\end{equation}
A deterministic sensitivity bound gives \(\|MV-MV'\|_F\le \|M\|\,\|\Delta V\|_F\). Using \(\|M\|\approx \sigma_M^2(\sqrt d+\sqrt r)^2\), we obtain
\begin{equation}
\label{eq:eps-class-mat-clean}
\varepsilon_{\mathrm{class}}^{(k)}
\;\le\;
\sigma_M^2(\sqrt d+\sqrt r)^2\,\sqrt{k}\,K_G,
\end{equation}
where $K_G \coloneqq \frac{\Delta_v}{\sigma_G}\sqrt{2\ln\!\Bigl(\frac{1.25}{\delta_G}\Bigr)} .$

By \Cref{thm:matrix-large-r-main} the $k$-column guarantee composes as
\begin{equation} \label{eq:eps-ours-k-clean}
\begin{aligned}
\varepsilon_{\mathrm{ours}}^{(k)} &= k(\varepsilon_\parallel+\varepsilon_\perp),
\;\text{ with } \\ \varepsilon_\parallel &\le \sigma_M^2(\sqrt d+\sqrt p)\sqrt p\,K_G,   
\end{aligned}
\end{equation}
where \(p=\dim(H)\le s\).

For comparison we set \(\delta_\parallel=\delta_G\). Combining~\Cref{eq:eps-class-mat-clean} and~\Cref{eq:eps-ours-k-clean} yields
\begin{equation}
\label{eq:ratio-decomp-clean}
\frac{\varepsilon_{\mathrm{ours}}^{(k)}}{\varepsilon_{\mathrm{class}}^{(k)}}
\;\le\;
\underbrace{\frac{k}{\sqrt{k}}\frac{(\sqrt d+\sqrt p)\sqrt p}{(\sqrt d+\sqrt r)^2}}_{\text{Gaussian part}}
\;+\;
\underbrace{\frac{k\,\varepsilon_\perp}{\sigma_M^2(\sqrt d+\sqrt r)^2\,\sqrt{k}\,K_G}}_{\text{residual part}} .
\end{equation}


We can further bound $\varepsilon_\perp$~(\Cref{lem:resid-dp}) 
\[
\varepsilon_\perp
\le
\underbrace{\frac{m-q+1}{2}\ln(\rho_\perp+\alpha)}_{T_1}
\;+\;
\underbrace{\frac{K}{2}\left(\frac{1}{\rho_\perp-\alpha}-1\right)}_{T_2}.
\]
where\(m=d-s\), \(q=r-p\) and
\[
\alpha \coloneqq \sqrt{\frac{1-\rho_\perp^2}{q}}\; t_q\!\left(1-\frac{\delta'}{3}\right),
\qquad
K \coloneqq \kappa_{m+q-1}\!\left(1-\frac{\delta'}{3}\right),
\]

In particular, when \(\rho_\perp\) is close to \(1\) and \(\alpha\) is small (e.g., for larger \(q\) and moderate \(\delta'\)), the residual part is small, so the comparison is dominated by the Gaussian part. Moreover in the rank-deficient regime $s<r$, we have $p=s$ a.s., so the Gaussian coefficient becomes
\begin{equation}
\label{eq:ratio-gauss-s<r-clean}
\frac{(\sqrt d+\sqrt s)\sqrt s}{(\sqrt d+\sqrt r)^2}.
\end{equation}
In this regime, our bound strictly improves on the classical baseline. For a more detailed discussion please see Appendix TODO.

==> icml2026/content/discussion.tex <==
\textbf{Related works} Random projections are widely exploited in the privacy literature. Some works, such as \citet{Kenthapadi2013JL,li2023signprojection}, explore the privacy of JL-style projections or random sign flipping. However, these approaches typically do not treat the projection’s randomness as part of the privacy mechanism: they publish the projection matrix and regard its randomness as public information. Other lines of work use projections mainly for dimensionality reduction to improve the privacy–utility trade-off by reducing the dimension dependence in convergence guarantees~\citep{jiang2025balancingrpsgd,kasiviswanathan21a,li2011compressive,or2019oldtechnique}. The intuition is similar to our~\Cref{thm:matrix-dp-proj-mechanism-small-r}, however, those results improve utility in expectation or with high probability over algorithmic randomness, whereas we directly establish a \emph{privacy amplification} at fixed noise and characterize its dependence on the rank \(r\).

Far fewer works exploit projection randomness itself as a privacy resource. ~\citet{lev2025the} show that Gaussian sketching can amplify privacy: releasing a Gaussian sketch with additive noise ($Z^\top V + \Xi$) yields improved privacy guarantees under a ''scale'' assumption on the singular values of the data matrix. Our setting is LoRA-motivated and geometrically different: we project with a Wishart matrix $M = ZZ^\top$ and release~$M V + \Xi$~(\ref{eq:M1}). As $M$ is PSD, the induced geometry differs from Gaussian sketching, leading to a different analysis and assumptions. Nevertheless, the takeaway is the same: intrinsic projection randomness plus modest noise can yield stronger privacy guarantees than additive noise alone.

There is also a line of work on privacy amplification via compression. In particular,~\citet{jin2025signsgd} shows that by compressing the gradient to their signs, amplifies privacy guarantees. Perhaps most related to our work, \citet{Hao2024Flora} interpret LoRA as gradient compression via (re-sampled) low-dimensional random projections, but their motivation is primarily \emph{efficiency}, not privacy. \citet{malekmohammadi2025lowrankadaptationsecretlyimitates} argue via a CLT-based approximation that LoRA can induce DP-SGD-like training dynamics for certain architectures in the limit. In contrast, we provide \emph{non-asymptotic} results for the finite-dimensional updates used in LoRA: we give formal differential privacy guarantees for vector valued updates, a sharp non-privacy result for noise-free matrix updates, and finally show that when adding small amounts of additive noise to the gradients the random projections yield \emph{privacy amplification} beyond noise calibration alone.

\textbf{Discussion} The negative result for matrix-valued updates shows that noise-free matrix-valued LoRA-FA updates are not differentially private. This worst-case statement does not preclude weaker privacy notions. Apart from this, in~\cref{tab:mia-noiseless} we observe perfect success for $r \geq 128$, but slightly lower success when $r$ is extremely small. We attribute this gap primarily to a utility effect: very small-r LoRA does not achieve comparable test accuracy, making loss-based MIA less sensitive. Understanding LoRA’s privacy risk under weaker adversaries, and disentangling genuine privacy gains from ineffective MIA adversaries at small $r$, is an interesting direction for future work.

On the positive side, we show that once additive noise is introduced, the intrinsic randomness of the projection mechanism can be leveraged to amplify privacy. However, for the large $r$ case~(\Cref{subsec:matproj-large-r}) these alignment-based guarantees rely on data-dependent properties that may be difficult to verify or enforce in practice. An interesting direction for future work is to design algorithms or training objectives that promote such alignment, or to exploit it when present to improve privacy--accuracy trade-offs.

% This work separates three regimes for Wishart-based random projections:
% (i) for vector-valued outputs, the Wishart projection mechanism admits formal \((\varepsilon,\delta)\)-DP guarantees;
% (ii) for matrix-valued outputs, the same intuition breaks down:without additive noise, the mechanism is not DP in general due to a geometric support mismatch; and
% (iii) once noise is added, the projection's intrinsic randomness can amplify Gaussian privacy.


% Perhaps most related to our work,~\citet{Hao2024Flora,malekmohammadi2025lowrankadaptationsecretlyimitates} argue that LoRA can be viewed as gradient compression through low-dimensional random projection and induces training dynamics resembling DP-SGD for certain architectures. 
% However, to our knowledge, we are the first to provide a formal differential privacy guarantee for compression achieved via random projection for arbitrary model choice. 

% Comparison to DP-LoRA and projected sgd??

==> icml2026/content/experiments.tex <==
The Gaussian baseline that ignores the randomness in \(M\) corresponds to standard DP-SGD: since \(V^\top=\nabla_W \cL(W_t)\), privatizing \(V\) directly (treating \(M\) as post-processing) amounts to adding Gaussian noise to the full gradient matrix, i.e., updating without any low-rank projection.

We emphasize that our mechanism \(\cA_2\) is not identical to the standard implementation of DP-LoRA-FA. In our analysis, we add Gaussian noise to \(V^\top=\nabla_W \cL(W_t)\) and then apply the random projection. In contrast, DP-LoRA-FA adds noise after first multiplying by \(A^\top\), i.e., to \(\nabla_W \cL(W_t)A^\top\). We focus on the former variant because it admits a more tractable theoretical analysis. Nonetheless, Appendix~\ref{app:subsec-comparison-dp-lora-small-r} shows that, with high probability, the two procedures inject noise of the same order. Moreover, our implementation does not require explicitly forming the full matrix gradient \(\nabla_W \cL(W_t)\): it can be realized using only gradients with respect to the trainable LoRA factor $B$~(\Cref{algo:lora-add-noise-1}), preserving the computational motivation of LoRA. For completeness, we include the standard DP-LoRA-FA implementation in our experiments.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.97\linewidth]{fig/dp_lora_vs_ours_plots.png}
    \caption{Comparison of DP-SGD, DP-LoRA, and our noisy LoRA~(\ref{eq:M2}) with our accounting method in~\Cref{thm:matrix-dp-proj-mechanism-small-r}}
    \label{fig:comparison}
\end{figure}
For an empirical comparison of these different methods, we fine-tune on CIFAR-10 to compare our method (\ref{eq:M2} with the privacy accounting from \Cref{thm:matrix-dp-proj-mechanism-small-r}) with DP-Lora-FA and DP-SGD under the same privacy budget.
Appendix~\ref{app:subsec-comparison-exp-details} provides implementation details (backbone, hyper-parameter grid, and accounting). 

\Cref{fig:comparison} (right) reports test accuracy as a function of the privacy budget $\varepsilon$ for $\delta = 10^{-4}$. In the small $\varepsilon$ regime, our method (and DP-LoRA at extremely low $\varepsilon$) outperforms DP-SGD, since the low-rank projection reduces the amount of noise required to achieve a given privacy level. \jd{is there a regime where our method outperform dp-sgd and dp-lora doesn't? if yes we should mention that no?} As $\varepsilon$ increases, the required noise decreases for all methods and this advantage diminishes. In the large $\varepsilon$ regime the accuracy gains from reduced noise are outweighed by the optimization bias introduced by the low-rank constraint, so DP-SGD matches or slightly outperforms our approach.

In~\Cref{fig:comparison} (left), we isolate the effect of the low-rank projection by comparing our method $\cA_2$ across ranks $r$ at a fixed privacy budget. While the two approaches are similar and, with high probability, add effective noise of the same order (see Appendix~\ref{app:subsec-comparison-dp-lora-small-r} for details), we observe that our Wishart projection is consistently better, especially at smaller ranks. This suggests that beyond the amount of injected noise, the geometry of the random projection (applied to both the gradient matrix and the noise) also affects model utility. Understanding when and why different projection distributions perform better remains an interesting direction for future work.


==> icml2026/content/intro.tex <==
Differential Privacy~(DP)~\citep{dwork2006calibrating} is widely regarded as the gold standard for protecting training data privacy in machine learning. Intuitively, DP limits the influence of any single example on the output, making it difficult to infer whether that example appeared in the training set. The most widely used DP algorithm in modern ML is DP-SGD~\citep{Abadi2016}, the private counterpart of the de facto standard optimization algorithm Stochastic Gradient Descent~(SGD). 

However, DP-SGD is computationally demanding and often incurs a substantial utility loss, especially for large models. While it remains one of the few viable choices for training machine learning models from scratch, in many practical deployments sensitive data enters primarily during fine-tuning, e.g. when an organization adapts a public pre-trained model on proprietary data. This motivates a simple strategy: start from a large public pre-trained model and enforce privacy only during fine-tuning. In the non-private setting, parameter-efficient fine-tuning (PEFT) \citep{han2024parameterefficient} updates only a small set of parameters while freezing the base model, substantially reducing memory and compute. This naturally raises the question: can PEFT similarly reduce the cost of DP fine-tuning?

\emph{Low-Rank Adaptation (LoRA)}~\citep{hu2022lora} is a widely used PEFT method that often matches full-parameter fine-tuning on downstream tasks~\citep{hu2022lora, dettmers2023qlora}. It freezes the pre-trained weights and inserts randomly initialised trainable low-rank matrices, dramatically shrinking the number of trainable parameters. Variants include adaptive-rank methods~\citep{zhang2023adalora}, quantization-aware tuning for low-bit backbones~\citep{dettmers2023qlora, li2023loftq}, stability/initialization refinements~\citep{hayou2024lora+, meng2024pissa}, and structural decompositions~\citep{liu2024dora}, each targeting better accuracy under tight compute and memory budgets. Approaches to privatising LoRA have also been proposed, including DP-LoRA~\citep{Liu2025}.

Several LoRA variants~\citep{sun2024improving, Hao2024Flora} already incorporate substantial randomness (e.g., repeated re-initialization of component weight matrices). Yet most privatisation algorithms treat LoRA updates as deterministic given the data and do not explicitly leverage this inherent randomness. At the same time, empirical studies report reduced memorisation under LoRA~\citep{hong2025evaluating} even without any explicit privatisation.


Following~\citet{Hao2024Flora}, we note that in certain LoRA variants (e.g. LoRA-FA~\citep{lorafa2023}, the update behaves as if it applies a random Wishart projection to the gradient. We formalize this behaviour through the following abstraction, (which allows us to rigorously analyse the privacy guarantee of these methods)

\begin{defn}[Projection mechanism]
    \label{defn:projection-mech}
    Let $\cS\subset\cX^n$  be a dataset collection and $f:\mathcal{S}\to\mathbb{R}^{n\times d}$ a query function.
    For $r\in\mathbb{N}$, the (Wishart) projection mechanism is defined by
    \[
    \mathcal{A}_{r}(S) \coloneqq f(S)M,
    \qquad
    M := Z^\top Z,
    \]
    where $Z\in\mathbb{R}^{r\times d}$ has i.i.d rows $z_k\overset{i.i.d}{\sim}\mathcal{N}\br{0,\frac{1}{r}I_d}$ or equivalently, $M\sim \mathsf{W}_d(\frac{1}{r}I_d,\,r)$\footnote{All of our analysis extends to Gaussian noise $Z\sim \cN(0, \sigma^2I_d)$ for any $\sigma^2 > 0$. We set $\sigma^2 = 1/r$ to match the usual normalization of Wishart random projection (e.g. in LoRA initializations). }.
\end{defn}
We therefore analyse $\mathcal{A}_{r}$ as a proxy for LoRA’s built-in randomness. Unlike the Johnson–Lindenstrauss~\citep{johnson1984extensions} transform, which is a random embedding that preserves norms, the Wishart projection is a random positive semidefinite reweighting that is isotropic in expectation but can distort norms in a single draw.


Recent work~\citep{malekmohammadi2025lowrankadaptationsecretlyimitates} conjectures that LoRA training dynamics may inherently possess privacy properties. Specifically, they show that individual rows of the gradient matrix asymptotically resembles the noise distribution of DP-SGD as the dimension $d\to \infty$. In contrast, we establish non-asymptotic differential privacy guarantees for the vector-valued projection mechanism in~\Cref{thm:vec-alt}. However, LoRA updates are matrix-valued: in our abstraction, they correspond to applying the projection mechanism to gradient matrices. We show that this matrix-valued projection mechanism, and hence LoRA, is not private in general~(\Cref{prop:neg-res}): in the setting without additional additive noise, neighbouring datasets can yield non-overlapping support, enabling (near) perfect membership inference with AUC $\geq 0.99$ as illustrated in~\Cref{tab:mia-noiseless}.
 
Nevertheless, LoRA’s built-in randomness is not irrelevant: it is simply insufficient on its own. We therefore consider a noisy variant of the projection mechanism, obtained by adding a small amount of additive noise. This enforces overlap for output distributions of neighbouring datasets, and the above attack no longer succeeds. In this setting we extend our guarantees from vectors to matrices and show that Wishart projection can amplify privacy. For fixed noise, composing with the projection yields strictly stronger privacy bounds than the noise level alone would suggest, both for large $r$~(\Cref{subsec:matproj-large-r}) and in the practically relevant small-$r$ regime~(\Cref{subsec:matproj-small-r}). A key implication is that low rank is beneficial beyond utility: at a fixed noise multiplier, projection can amplify privacy and yield smaller $\varepsilon$ than full fine-tuning, a point not made explicit in prior DP-LoRA analyses.

We summarize our contributions below. 
\begin{enumerate}[label=(\roman*)]
    %\renewcommand{\labelenumi}{(\roman{enumi})}
    \item We introduce the Wishart projection mechanism and prove non-asymptotic DP guarantees in the vector case. 
    \item We show the corresponding matrix mechanism is not DP, and demonstrate its vulnerability via a near-perfect MIA (AUC $> 0.99$).
    \item For a variant involving additive noise, we prove privacy amplification for both large and small ranks.
\end{enumerate}

\noindent\textbf{Organization.} In~\Cref{sec:prelim} we review DP preliminaries and give a brief overview of why LoRA is an instance of the Wishart projection mechanism.~\Cref{sec:proj-mechanism-vector} proves privacy for vector-valued functions and shows why it fails for matrices.~\Cref{sec:proj-mechanism-matrix} analyses the noisy Wishart projection mechanism for matrix-valued functions and establishes privacy amplification in both rank regimes. Finally,~\Cref{sec:discussion} covers related work, limitations, and open questions.

==> icml2026/content/matproj.tex <==
%!TEX root = ../iclm2026.tex

As shown in the previous section, the symmetry constraint induced by a Wishart (PSD) projection can make the output supports of neighboring matrix inputs disjoint. This motivates adding a small amount of Gaussian noise to enforce overlap if we want to keep DP guarantee. 

In this section, we show that once overlap exists, the intrinsic randomness of the Wishart projection can
amplify privacy beyond what an analysis based on additive noise alone would suggest.
We study two noisy variants (\ref{eq:M1} and~\ref{eq:M2}), and distinguish two complementary amplification mechanisms:
(i) a large-rank phenomenon~(\Cref{subsec:matproj-large-r}) driven by posterior-stable residual randomness in $M$;
and (ii) a small-rank phenomenon~(\Cref{subsec:matproj-small-r}) given by random subspace hiding.


\noindent\textbf{Setup and Mechanism. }
Let \(d,n,r\ge 1\) and fix the noise scale \(\sigma_G>0\). Draw \(Z\in\mathbb{R}^{d\times r}\) with i.i.d.\ entries \(Z_{ik}\sim\mathcal{N}(0,1/r)\) and set \(M:=ZZ^\top\in\mathbb{R}^{d\times d}\). Let \(\Xi \coloneqq [\xi_1,\ldots,\xi_n]\in\mathbb{R}^{d\times n}\) with i.i.d columns \(\xi_k\sim\mathcal{N}(0,\sigma_G^2 I_d)\).
\begin{defn}[Noisy Projection Mechanisms]
Given $V=\bs{v_1,\dots,v_n}\in\bR^{d\times n}$, define\footnote{We adopt left-multiplication in \ref{eq:M1} and \ref{eq:M2} for analytical convenience, but they have the identical privacy guarantee as~\Cref{defn:projection-mech}. }:
\begin{align}
\cA_1(V) &\coloneqq MV+\Xi \tag{M1}\label{eq:M1}\\
\cA_2(V) &\coloneqq M(V+\Xi) \tag{M2}\label{eq:M2}
\end{align}
\end{defn}

\subsection{Matrix Projection in the large $r$ regime}\label{subsec:matproj-large-r}
\input{content/matproj_large_r_v2}
%\input{content/matproj_gaussian_comp}
\subsection{Matrix Projection in the small $r$ regime}\label{subsec:matproj-small-r}
\input{content/matproj_small_r_v2}

==> icml2026/content/matproj_gaussian_comp.tex <==
\subsubsection{Comparison with the Classical Gaussian Mechanism}\label{subsec:compare-classical}
\as{Have not edited below}
We next compare the privacy guarantee in \Cref{thm:matrix-large-r-main} to a classical baseline that ignores the intrinsic randomness in $M$. The baseline treats $V\mapsto MV$ as deterministic, applying the Gaussian mechanism calibrated to the Frobenius sensitivity.


\noindent\textbf{Setup.}
Fix \(V,V'\in\mathbb{R}^{d\times n}\). Let \(J=J(V,V')\) with \(k \coloneqq |J|\). Assume \(\|v_j\|_2=\|v'_j\|_2=1\) and \(\|v_j-v'_j\|_2\le \Delta_v\) for all \(j\in J\) (e.g., \Cref{eq:Deltav}), then
\begin{equation}
\label{eq:DV-frob-cmpr}
\|\Delta V\|_F^2=\sum_{j\in J}\|v_j-v'_j\|_2^2 \le k\Delta_v^2.
\end{equation}
A deterministic sensitivity bound gives \(\|MV-MV'\|_F\le \|M\|\,\|\Delta V\|_F\). Using \(\|M\|\approx \sigma_M^2(\sqrt d+\sqrt r)^2\), we obtain
\begin{equation}
\label{eq:eps-class-mat-clean}
\varepsilon_{\mathrm{class}}^{(k)}
\;\le\;
\sigma_M^2(\sqrt d+\sqrt r)^2\,\sqrt{k}\,K_G,
\end{equation}
where $K_G \coloneqq \frac{\Delta_v}{\sigma_G}\sqrt{2\ln\!\Bigl(\frac{1.25}{\delta_G}\Bigr)} .$

By \Cref{thm:matrix-large-r-main} the $k$-column guarantee composes as
\begin{equation} \label{eq:eps-ours-k-clean}
\begin{aligned}
\varepsilon_{\mathrm{ours}}^{(k)} &= k(\varepsilon_\parallel+\varepsilon_\perp),
\;\text{ with } \\ \varepsilon_\parallel &\le \sigma_M^2(\sqrt d+\sqrt p)\sqrt p\,K_G,   
\end{aligned}
\end{equation}
where \(p=\dim(H)\le s\).

For comparison we set \(\delta_\parallel=\delta_G\). Combining~\Cref{eq:eps-class-mat-clean} and~\Cref{eq:eps-ours-k-clean} yields
\begin{equation}
\label{eq:ratio-decomp-clean}
\frac{\varepsilon_{\mathrm{ours}}^{(k)}}{\varepsilon_{\mathrm{class}}^{(k)}}
\;\le\;
\underbrace{\frac{k}{\sqrt{k}}\frac{(\sqrt d+\sqrt p)\sqrt p}{(\sqrt d+\sqrt r)^2}}_{\text{Gaussian part}}
\;+\;
\underbrace{\frac{k\,\varepsilon_\perp}{\sigma_M^2(\sqrt d+\sqrt r)^2\,\sqrt{k}\,K_G}}_{\text{residual part}} .
\end{equation}


We can further bound $\varepsilon_\perp$~(\Cref{lem:resid-dp}) 
\[
\varepsilon_\perp
\le
\underbrace{\frac{m-q+1}{2}\ln(\rho_\perp+\alpha)}_{T_1}
\;+\;
\underbrace{\frac{K}{2}\left(\frac{1}{\rho_\perp-\alpha}-1\right)}_{T_2}.
\]
where\(m=d-s\), \(q=r-p\) and
\[
\alpha \coloneqq \sqrt{\frac{1-\rho_\perp^2}{q}}\; t_q\!\left(1-\frac{\delta'}{3}\right),
\qquad
K \coloneqq \kappa_{m+q-1}\!\left(1-\frac{\delta'}{3}\right),
\]

In particular, when \(\rho_\perp\) is close to \(1\) and \(\alpha\) is small (e.g., for larger \(q\) and moderate \(\delta'\)), the residual part is small, so the comparison is dominated by the Gaussian part. Moreover in the rank-deficient regime $s<r$, we have $p=s$ a.s., so the Gaussian coefficient becomes
\begin{equation}
\label{eq:ratio-gauss-s<r-clean}
\frac{(\sqrt d+\sqrt s)\sqrt s}{(\sqrt d+\sqrt r)^2}.
\end{equation}
In this regime, our bound strictly improves on the classical baseline. For a more detailed discussion please see Appendix TODO.

==> icml2026/content/matproj_large_r_v2.tex <==
% !TeX root = ../icml_main.tex

We first study the mechanism \(\cA_1(V)=MV+\Xi\)~(\ref{eq:M1}). Unlike the vector case, privacy can fail even when only one column of $V$ changes. The issue is that the same random matrix \(M\) is reused across columns: after observing \(n-1\) columns, an adversary can learn information about \(M\) and use it to infer the remaining column more accurately. Thus additive noise \(\Xi\) is needed to mask this leakage and ensure distributional overlap.

\subsubsection{Setting and Main Theorem} We first prove a privacy guarantee for a one-column adjacency, and then lift it to a more general matrix adjacency by composing such one-columns steps. Before stating our results, we define these adjacency relations in~\Cref{def:adj-matrix}.
% Our privacy guarantee is stated for a matrix-level notion of adjacency. Informally, we compare \(V\) and
% \(V'\) by changing one column at a time.  When we change column
% \(j\), we measure the change relative to the subspace spanned by the
% other columns, since that subspace is already revealed by the rest of
% the release. This leads to a one-column adjacency relation, and a
% matrix adjacency relation obtained by composing such one-column steps.

Throughout this section we assume all columns are unit vectors:
\(\|v_j\|_2=\|v'_j\|_2=1\).  For \(V,V'\in\R^{d\times n}\), write
\(J(V,V') \coloneqq \{j\in[n]: v_j\neq v'_j\}\), and for any
\(j\in[n]\), let \(V_{-j}\) denote \(V\) with column \(j\) removed.

\begin{defn}[Adjacency notion]
\label{def:adj-matrix}
Fix parameters \(\beta_\perp\in[0,1]\) and
\(\rho_\parallel,\rho_\perp\in[-1,1]\).
\begin{enumerate}[leftmargin=*, itemsep=2pt, topsep=2pt, parsep=0pt, partopsep=0pt]
\item \textbf{(One-column adjacency).} Fix \(j\in[n]\) and set \(S\coloneqq \mathrm{span}(V_{-j})\subset\R^d\).
We write \(V\sim_A^{(j)}V'\) if \(V_{-j}=V'_{-j}\) and, writing
\(v_j=a+b\) and \(v'_j=a'+b'\) with \(a,a'\in S\) and \(b,b'\in S^\perp\), we have
\[
\norm{b}_2,\norm{b'}_2=\beta_\perp,~
\frac{\ip{a}{a'}}{\norm{a}_2\norm{a'}_2}\ge \rho_\parallel,~
\frac{\ip{b}{b'}}{\norm{b}_2\norm{b'}_2}\ge \rho_\perp.
\]

\item \textbf{(Matrix adjacency).} We write \(V\sim_A V'\) if there
exists an ordering \(j_1,\dots,j_k\) of \(J(V,V')\) where \(k = \abs{J(V,V')} \),
matrices \(V^{(0)},\dots,V^{(k)}\) such that \(V^{(0)}=V\),
\(V^{(k)}=V'\), and \(V^{(t-1)}\sim_A^{(j_t)} V^{(t)}\) for all
\(t\in[k]\).
\end{enumerate}
\end{defn}

The parameter \(\beta_\perp\) measures how much of the changed column
lies outside the span exposed by the other columns. The parameters
\(\rho_\parallel\) and \(\rho_\perp\) control alignment within \(S\)
and \(S^\perp\), respectively.

\begin{thm}[Privacy of~\ref{eq:M1} in the large-$r$ regime]
\label{thm:matrix-large-r-main}
Fix \(\beta_\perp,\rho_\parallel,\rho_\perp\) and let \(V\sim_A V'\) with \(k=|J(V,V')|\). Define \((\varepsilon_{\mathrm{one}},\delta_{\mathrm{one}})\)
as the privacy parameters for a single admissible step \(V\sim_A^{(j)}V'\)
(given in \Cref{thm:matrix-onecol-directional}).
Then \(\cA_1\) is \((\varepsilon,\delta)\)-DP for inputs \(V,V'\), with
\[
\varepsilon \le k\,\varepsilon_{\mathrm{one}},
\qquad
\delta \le k\,e^{(k-1)\varepsilon_{\mathrm{one}}}\,\delta_{\mathrm{one}}.
\]
\end{thm}

\subsubsection{Proof Sketch}
Let \(V^{(0)},\dots,V^{(k)}\) be the adjacency chain from \Cref{def:adj-matrix}. As in group privacy, it suffices to prove a privacy guarantee for a single step where only one column changes, and then use a group-privacy style analysis to compose those guarantees along the chain. So the main work is the one-column case
% We first prove a one-column guarantee for \(\cA_1\) under
% \(V^{(t-1)}\sim_A^{(j_t)}V^{(t)}\), and then compose these bounds along the chain proceeding in a similar fashion to the standard DP group-privacy proof. Thus, the main work is the one-column analysis.

Fix a step \(V\sim_A^{(j)}V'\). The matrices agree on all columns except $j$ so \(V_{-j}=V'_{-j}\). Write the mechanism's output as:
\[
(X,Y)\coloneqq \bigl(Mv_j+\xi_j,\; MV_{-j}+\Xi_{-j}\bigr).
\]
Let \(S=\mathrm{span}(V_{-j})\) with orthonormal basis \(U\), and set \(G\coloneqq U^\top Z\).
Using the decomposition \(M=M_\parallel+M_\perp\) from Appendix~\ref{app:matrix-large-r}, we have:
(i) \(M_\perp V_{-j}=0\), so \(Y\) depends only on \(M_\parallel\); and
(ii) \emph{posterior stability}: conditional on \(G\), the residual block \(M_\perp\) remains independent of \(Y\).
This is the key decoupling: after observing the unchanged columns, the randomness in \(M_\perp\) is still ``fresh''.

Decompose \(v_j=a+b\) and \(v_j'=a'+b'\) with \(a,a'\in S\) and \(b,b'\in S^\perp\).
Since \(M_\perp a=0\), the released column splits as
\[
Mv_j+\xi_j
=\underbrace{(M_\parallel v_j+\xi_j)}_{=:C(v_j)}
+\underbrace{M_\perp b}_{=:R(b)} .
\]
We bound these two parts separately and then compose.
\noindent\textbf{Residual term. }For the residual term \(R(b)\), posterior stability~(\Cref{lem:posterior-stable}) lets us apply the \emph{vector-valued} DP analysis from \Cref{sec:proj-mechanism-vector}, yielding an \((\varepsilon_\perp,\delta_\perp)\) bound. Let
\(\Phi\) be the standard normal CDF; let \(t_q\) and \(\kappa_\ell\)  be the quantiles of Student $t$ and $\chi_\ell^2$ distributions, respectively. 

\begin{restatable}[Residual DP
bound]{lem}{privrescomponent}\label{lem:resid-dp} 

Write \(s\coloneqq \dim(S)\) and \(m\coloneqq d-s\). Fix
\(\rho_\perp\in(0,1]\) and \(\delta'\in(0,1)\), and define
\[
K_\perp = \sqrt{\tfrac{1-\rho_\perp^2}{q}}t_q\br{1-\nicefrac{\delta'}{3}}, 
\]
Then the residual release \(R(b)=M_\perp b\) is
\((\varepsilon_\perp,\delta_\perp)\)-DP for inputs \(b,b'\)
satisfying~\Cref{def:adj-matrix} where
\[
\delta_\perp
=\E_{X\sim\chi^2_q}\bs{\Phi\br{-\tfrac{\rho_\perp\sqrt{X}}{\sqrt{1-\rho_\perp^2}}}}+\delta',\]\[\varepsilon_\perp
\le
\tfrac{m-q+1}{2}\ln(\rho_\perp+K_\perp)
+\frac{\kappa_{m+q-1}\br{1-\nicefrac{\delta'}{3}}}{2}\left(\tfrac{1}{\rho_\perp-K_\perp}-1\right).  \] 
\end{restatable}


\noindent\textbf{Correlated term. }For the correlated term \(C(v_j)\), we apply the Gaussian mechanism with a high-probability directional sensitivity bound for \(M_\parallel\):
with probability at least \(1-\delta_s\) over \(Z\),
\(
\|M_\parallel(v_j-v'_j)\|_2 \le \Gamma_{\delta_s}\|v_j-v'_j\|_2
\)
(\Cref{lem:dir-bound}).
% and  using 
% \begin{equation}
% \label{eq:Deltav}
% \begin{aligned}
% \Delta_v^2
% &\coloneqq \max_{V\sim_A^{(j)}V'} \|v_j-v'_j\|_2^2
% =\|a-a'\|_2^2+\|b-b'\|_2^2 \\
% &\le 2\Bigl((1-\beta_\perp^2)(1-\rho_\parallel)+\beta_\perp^2(1-\rho_\perp)\Bigr).
% \end{aligned}
% \end{equation}
Conditioning on this event we get the correlated term is \(
(\varepsilon_\parallel,\delta_\parallel)-DP
\)
with 
\begin{equation}\label{eq:eps-parallel-mat}    
\varepsilon_\parallel
\coloneqq
\frac{\Gamma_{\delta_s}\Delta_v}{\sigma_G}\sqrt{2\ln\br{\nicefrac{1.25}{\delta_\parallel}}}.
\end{equation}

Finally, sequential composition gives
\(
\varepsilon_{\mathrm{one}}\le \varepsilon_\parallel+\varepsilon_\perp
\)
and
\(
\delta_{\mathrm{one}}\le \delta_\parallel+\delta_\perp+\delta_s.
\)
\begin{restatable}{thm}{privmatrixprojonecol}\label{thm:matrix-onecol-directional}
Fix $j\in[n]$. Let $V\sim_A^{(j)}V'$ with parameters $(\rho_\parallel,\beta_\perp,\rho_\perp)$ defined in~\Cref{def:adj-matrix}.
Fix $\delta_\parallel,\delta_s\in(0,1)$, and choose $\delta'>0$ as in \Cref{lem:resid-dp} to obtain $(\varepsilon_\perp,\delta_\perp)$.
Let $p=\mathrm{rank}(U^\top Z)$ and define $\Gamma_{\delta_s}$ as
above, and \(\varepsilon_\parallel\) as in \Cref{eq:eps-parallel-mat}.
Then the mechanism $\cA_1(V)=MV+\Xi$ is $(\varepsilon_{\mathrm{one} },\delta_{\mathrm{one} })$-DP for inputs $V\sim_A^{(j)}V'$, with
\[
\varepsilon_{\mathrm{one} } \le \varepsilon_\parallel+\varepsilon_\perp,
\qquad
\delta_{\mathrm{one} }\le \delta_\parallel+\delta_\perp+\delta_s.
\]
\end{restatable}
Composing the one-column bounds along the chain yields \Cref{thm:matrix-large-r-main}.



% Let
% \(S=\mathrm{span}(V_{-j})\) with orthonormal basis \(U\in\R^{d\times
% s}\), and set \(G\coloneqq U^\top Z\). Then, write the output as
% \(\cA_1(V)=(X,Y)\), where \( \br{X,Y}\coloneqq\br{Mv_j+\xi_j,~
% MV_{-j}+\Xi_{-j}}.  \) 

% Using the exact decomposition \(M=M_\parallel+M_\perp\)~(details in
% \Cref{app:matrix-large-r}), we have two structural properties: (i)
% \(M_\perp V_{-j}=0\), hence \(Y\) depends only on \(M_\parallel\); and
% (ii) \emph{posterior stability}: conditional on \(G\), the residual
% block \(M_\perp\) remains independent of \(Y\). Now decompose
% \(v_j=a+b\) and \(v'_j=a'+b'\) with \(a,a'\in S\) and \(b,b'\in
% S^\perp\).  Since \(M_\perp a=0\), \(X\) splits as
% \[
% X
% = Mv_j+\xi_j
% = \underbrace{\br{M_\parallel v_j+\xi_j}}_{=:C(v_j)}
% +
% \underbrace{\br{M_\perp b}}_{=:R(b)}.
% \]
% We bound \(R(b)\) using the vector-case analysis
% from~\Cref{sec:proj-mechanism-vector}, and we bound \(C(v_j)\) using a
% Gaussian mechanism argument with a high-probability \emph{directional}
% sensitivity bound for \(M_\parallel\).


% First, we control the residual term \(R(b)\).  Let
% \(p=\mathrm{rank}(G)\le \min\{s,r\}\) and \(q=r-p\).  The following
% result gives \((\varepsilon_\perp,\delta_\perp)\)-DP for the residual
% release \(R(b)\) and follows immediately from \Cref{thm:vec-alt}.



% Next, we control the correlated term \(C\br{v_j}\). Under
% \Cref{def:adj-matrix} and orthogonality of \(S\) and \(S^\perp\), we
% have
% \begin{equation}
% \label{eq:Deltav}
% \begin{aligned}
% \Delta_v^2
% &\coloneqq \max_{V\sim_A^{(j)}V'} \|v_j-v'_j\|_2^2
% =\|a-a'\|_2^2+\|b-b'\|_2^2 \\
% &\le 2\Bigl((1-\beta_\perp^2)(1-\rho_\parallel)+\beta_\perp^2(1-\rho_\perp)\Bigr).
% \end{aligned}
% \end{equation}
% To apply the Gaussian mechanism to \(C(v_j)=M_\parallel v_j+\xi_j\),
% we need an upper bound on \(\norm{M_\parallel(v_j-v'_j)}_2\).  We use
% a directional bound shown in \Cref{lem:dir-bound}: with probability at
% least \(1-\delta_s\) over the draw of \(Z\),
% \[
% \norm{M_\parallel(v_j-v'_j)}_2 \le \Gamma_{\delta_s}\,\norm{v_j-v'_j}_2,
% \]
% where
% \(
% \Gamma_{\delta_s}\coloneqq \sigma_M^2\br{\sqrt d+\sqrt p+g_{\delta_s}}\br{\sqrt p+g_{\delta_s}},\) and \(g_{\delta_s}=\sqrt{2\ln(2/\delta_s)}.\) For comparison, the crude bound \(\norm{M_\parallel(v_j-v'_j)} \le \norm{M_\parallel} \norm{v_j-v'_j}\),
% together with \(\norm{M_\parallel}\lesssim \sigma_M^2\br{\sqrt
% d+\sqrt p+g_{\delta_s}}^2,\) is strictly looser.

% Conditioning on the event \(\norm{M_\parallel(v_j-v'_j)} \le
% \Gamma_{\delta_s}\norm{v_j-v'_j}\), the Gaussian mechanism with noise
% \(\xi_j\sim \cN(0,\sigma_G^2 I_d)\) yields
% \begin{equation}\label{eq:eps-parallel-mat}    
% \varepsilon_\parallel
% \coloneqq
% \frac{\Gamma_{\delta_s}\Delta_v}{\sigma_G}\sqrt{2\ln\br{\nicefrac{1.25}{\delta_\parallel}}}.
% \end{equation}
% We combine the residual guarantee and the Gaussian-mechanism guarantee
% by sequential composition, and then account for the sensitivity-tail
% event by adding \(\delta_s\) to the failure probability.  This yields
% the following one-column statement.



% Finally, \Cref{thm:matrix-large-r-main} follows by composing the bounds along the chain witnessing
% \(V\sim_A V'\) similar to the standard group-privay proof.

\subsubsection{Comparison with the Gaussian Mechanism}\label{subsec:compare-classical}
We next compare the privacy guarantee in \Cref{thm:matrix-large-r-main} to a classical baseline that ignores the randomness in $M$: it treats $V\mapsto MV$ as deterministic and applies the Gaussian mechanism calibrated to the Frobenius sensitivity.

Fix \(V,V'\in\mathbb{R}^{d\times n}\). Let \(J=J(V,V')\) with \(k \coloneqq |J|\). Assume \(\|v_j\|_2=\|v'_j\|_2=1\) and \(\|v_j-v'_j\|_2\le \Delta_v\) for all \(j\in J\), then
\begin{equation}
\label{eq:DV-frob-cmpr}
\|\Delta V\|_F^2=\sum_{j\in J}\|v_j-v'_j\|_2^2 \le k\Delta_v^2.
\end{equation}
A deterministic sensitivity bound gives \(\|MV-MV'\|_F\le \|M\|\,\|\Delta V\|_F\). Using \(\|M\|\approx \sigma_M^2(\sqrt d+\sqrt r)^2\), we obtain
\begin{equation}
\label{eq:eps-class-mat-clean}
\varepsilon_{\mathrm{class}}^{(k)}
\;\le\;
\sigma_M^2(\sqrt d+\sqrt r)^2\,\sqrt{k}\,K_G,
\end{equation}
where $K_G \coloneqq \frac{\Delta_v}{\sigma_G}\sqrt{2\ln\!\Bigl(\frac{1.25}{\delta_G}\Bigr)} .$ By \Cref{thm:matrix-large-r-main}, the $k$-column guarantee composes as
\begin{equation} \label{eq:eps-ours-k-clean}
\varepsilon_{\mathrm{ours}}^{(k)} = k(\varepsilon_\parallel+\varepsilon_\perp),
\text{ with }  \varepsilon_\parallel \le \sigma_M^2(\sqrt d+\sqrt p)\sqrt p\,K_G,   
\end{equation}
where \(p\le s\) is the effective dimension of the revealed column-span seen through the random projection (formally \(p=\mathrm{rank}(U^\top Z)\)), and \(s=\dim(S)\) with \(S=\mathrm{span}(V_{-j})\).

For comparison, we set \(\delta_\parallel=\nicefrac{\delta_G}{3}\). Combining~\Cref{eq:eps-class-mat-clean} and~\Cref{eq:eps-ours-k-clean} yields
\begin{equation}
\label{eq:ratio-decomp-clean}
\frac{\varepsilon_{\mathrm{ours}}^{(k)}}{\varepsilon_{\mathrm{class}}^{(k)}}
\;\le\; \sqrt{k} \left(
\underbrace{\frac{(\sqrt d+\sqrt p)\sqrt p}{(\sqrt d+\sqrt r)^2}}_{\text{Gaussian part}}
\;+\;
\underbrace{\frac{\varepsilon_\perp}{\sigma_M^2(\sqrt d+\sqrt r)^2\,K_G}}_{\text{residual part}} \right).
\end{equation}


We can further bound $\varepsilon_\perp$ by~\Cref{lem:resid-dp}, 
\[
\varepsilon_\perp
\le
\underbrace{\frac{m-q+1}{2}\ln(\rho_\perp+\alpha)}_{T_1}
\;+\;
\underbrace{\frac{K}{2}\left(\frac{1}{\rho_\perp-\alpha}-1\right)}_{T_2}.
\]
where \(m=d-s\), \(q=r-p\) and \(\alpha\) and \(K\) are the \((1-\delta'/3)\)-quantiles defined in \Cref{lem:resid-dp}.
% \[
% \alpha \coloneqq \sqrt{\frac{1-\rho_\perp^2}{q}}\; t_q\!\left(1-\frac{\delta'}{3}\right),
% \qquad
% K \coloneqq \kappa_{m+q-1}\!\left(1-\frac{\delta'}{3}\right),
% \]

In particular, when \(\rho_\perp\) is close to \(1\) and \(\alpha\) is small (e.g., for larger \(q\) and moderate \(\delta'\)), the residual part is small, so the comparison is dominated by the Gaussian part. In the rank-deficient regime $s<r$, we moreover have $p=s$ a.s., so the Gaussian coefficient simplifies to
\begin{equation}
\label{eq:ratio-gauss-s<r-clean}
\frac{(\sqrt d+\sqrt s)\sqrt s}{(\sqrt d+\sqrt r)^2}.
\end{equation}
In this regime, the coefficient is $<1$, so our bound improves on the classical baseline. 
% For a more detailed discussion please see Appendix TODO.

==> icml2026/content/matproj_small_r_v2.tex <==
The small-\(r\) regime yields privacy amplification through a
different mechanism from the large $r$ regime. Here we analyse
\(\cA_2(V)=M(V+\Xi)\)~(\ref{eq:M2}). One might naively treat \(M\) as
post-processing: add Gaussian noise \(\Xi\) calibrated to the
Frobenius sensitivity~\(\|\Delta V\|_F\), then multiply by \(M\).
However, the important observation is that the output of $\cA_2$ always lies in the random column space \(\mathrm{col}\br{M}=\mathrm{col}\br{Z}\).
Consequently, conditioned on \(M\), privacy depends only on the
projected difference \(P_M\Delta V\), where \(P_M\) is the orthogonal
projector onto \(\mathrm{col}\br{M}\). When \(r\ll d\) the
projection typically captures only a small fraction of
\(\|\Delta V\|_F\), reducing the effective sensitivity. In rare
alignment events where \(\Delta V \approx P_M \Delta V\) the
amplification disappears and the guarantee becomes comparable to the naive approach.

\subsubsection{Main Theorem}


For \(V,V'\in\R^{d\times n}\) write \(\Delta V\coloneqq V-V'\).
For \(\varepsilon>0\) and \(\mu\ge 0\), define the Gaussian two-sided
tail function
\[
T(\varepsilon;\mu)
\coloneqq
\Phi\!\left(\frac{-\varepsilon+\mu/2}{\sqrt{\mu}}\right)
+
1-\Phi\!\left(\frac{\varepsilon+\mu/2}{\sqrt{\mu}}\right),
\]
where \(\Phi\) is the standard normal CDF and
\(T(\varepsilon;0)=0\).

\begin{restatable}[Privacy of \ref{eq:M2} in the small $r$-regime]{thm}{smallrmatrixdpprojmech}
\label{thm:matrix-dp-proj-mechanism-small-r}
Fix \(V,V'\in\R^{d\times n}\) and write \(s=\min\br{n,d}\). Then for
any \(\alpha\in(0,1)\) and any \(\varepsilon>0\), the mechanism
\(\cA_2\) is \(\br{\varepsilon,\delta_\alpha(\varepsilon)}\)-DP with
\[
\delta_\alpha(\varepsilon)
\le T\br{\varepsilon;\frac{\alpha\norm{\Delta V}_F^{2}}{\sigma_G^{2}}}
+
s\bs{1 - I_{\alpha}\br{\frac{r}{2},\frac{d-r}{2}}},
\]
where \(I_\alpha(a,b)\) is the regularized incomplete Beta function
(i.e.\ \(I_\alpha(a,b)=\Pr\bs{B\le \alpha}\) for
\(B\sim\mathrm{Beta}(a,b)\)).
\end{restatable}


\subsubsection{Proof Sketch}

Fix \(V,V'\) and condition on \(M\). Let \(P_M\) denote the orthogonal
projector onto \(\mathrm{col}(M)\). Conditioned on \(M\), the output $M(V + E)$
is a Gaussian matrix but supported on the rank-\(r\) subspace
\(\mathrm{col}(M)\). Consequently, the privacy loss depends on
\(\Delta V\) only through its projection onto \(\mathrm{col}(M)\),
namely \(\norm{P_M\Delta V}_F\). Let \(P\br{\cdot\mid M}\) and \(Q\br{\cdot\mid M}\) be the conditional
output laws under inputs \(V\) and \(V'\), respectively. Since
$\sigma_G > 0$ we have $P\br{\cdot \mid M} \ll Q\br{\cdot\mid M}$, so
we can define the conditional privacy loss random variable
\[
L_M(Y)\;\coloneqq\;\log\frac{dP\br{\cdot\mid M}}{dQ\br{\cdot\mid M}}(Y),
\quad Y\sim P\br{\cdot\mid M}.
\]
Then as shown in \Cref{lem:conditional-priv-loss} we have,
\[
L_M(Y)\sim
\cN\br{-\tfrac{\norm{P_M\Delta V}_F^2}{2\sigma_G^2},
\tfrac{\norm{P_M\Delta V}_F^2}{\sigma_G^2}}.
\]
This motivates the following good-projection event
\[
\cG_\alpha
\coloneqq
\bc{M: \norm{P_M\Delta V}_F^2\le \alpha\norm{\Delta V}_F^2},
\quad 0<\alpha<1.
\]

On the good event \(\cG_\alpha\), $L_M(Y)$ has a Gaussian tail:
\begin{equation}
\label{eq:gaussian-tail-small-r}
\Pr\br{\abs{L_M(Y)}>\varepsilon \mid M}
\le
T\br{\varepsilon;\tfrac{\alpha\norm{\Delta V}_F^2}{\sigma_G^2}}.
\end{equation}
Thus the unconditional $\delta$ is the Gaussian tail on $\cG_\alpha$ plus the failure probability  \(\Pr\br{\cG_\alpha^c}\). It remains to bound \(\Pr\br{\cG_\alpha^c}\).

Let \(\text{rank}(\Delta V) = s\), and let \(u_1,\dots,u_{s}\in\R^d\) be an orthonormal basis for \(\mathrm{col}\br{\Delta V}\). If \(\norm{P_M u_i}_2^2\le \alpha\) for all \(i\in\bs{s}\), then
\(
\norm{P_M\Delta V}_F^2 \le \alpha\norm{\Delta V}_F^2
\). Thus, the bad event \(\cG_\alpha^c\) implies \(\norm{P_M u_i}_2^2>\alpha\) for some
\(i\). Hence, by a union bound,
\[
\Pr(\cG_\alpha^c)
\le
 \sum_{i=1}^s \Pr\br{\norm{P_M u_i}_2^2>\alpha}.
\]
Since \(M=ZZ^\top\) with \(Z\in\R^{d\times r}\) Gaussian, \(\mathrm{col}(M)=\mathrm{col}(Z)\) is a random Haar rank-\(r\) subspace of \(\R^d\), and \(P_M\) is the orthogonal projector onto this
subspace~(\Cref{lem:delta-M-bound}).  For a fixed unit vector \(u\in\R^d\), the captured energy
\(\|P_Mu\|_2^2\) then follows the Beta law \(\mathrm{Beta}\!\br{\tfrac
r2,\tfrac{d-r}{2}}\). Therefore,
\[
\Pr\br{\cG_\alpha^c}
\le
s\bs{1 - I_{\alpha}\br{\frac{r}{2},\frac{d-r}{2}}}.
\]
Combining this with \eqref{eq:gaussian-tail-small-r} yields \Cref{thm:matrix-dp-proj-mechanism-small-r}.

\subsubsection{Comparison with the Gaussian Mechanism}
% \yh{We need to mention~\Cref{fig:small-r-privacy-amplification} somewhere; and maybe add another line with a smaller $r = 10$ to show our guarantee improves with smaller r. }
Without conditioning on \(M\), the standard Gaussian analysis uses sensitivity \(\|\Delta V\|_F\) and gives, for any $\varepsilon>0$,
\begin{equation}\label{equ:gauss-delta-small-r}
\delta_{\mathrm{Gauss}}(\varepsilon)
\;=\; T\!\left(\varepsilon;\frac{\|\Delta V\|_F^2}{\sigma^2}\right).
\end{equation}
This is robust but pessimistic, as it treats the full gap $\|\Delta V\|_F$ as visible. Conditioning on $M$ yields a tighter bound: \Cref{thm:matrix-dp-proj-mechanism-small-r} splits $\delta$ into a Gaussian term on the good event \(\mathcal{G}_\alpha\) and a failure probability:
\[
\delta_{\mathrm{ours}}(\varepsilon)
\;\le\;
T\!\left(\varepsilon;\,\frac{\alpha\|\Delta V\|_F^2}{\sigma^2}\right)
\;+\;
s\!\left[1 - I_{\alpha}\!\left(\frac{r}{2},\,\frac{d-r}{2}\right)\right].
\]
% \begin{wrapfigure}{r}[-10pt]{0.53\linewidth}
%     \vspace{-5pt}
%     \centering
%     \includegraphics[width=\linewidth]{fig/eps_vs_sigma_r10_r50_new.png}
%     \caption{Privacy loss $\varepsilon$ v.s. noise scale $\sigma$ for $\delta = 10^{-5}$, $d = 2000$: our bound~(\Cref{thm:matrix-dp-proj-mechanism-small-r}), optimized over $\alpha$ compared to~\Cref{equ:gauss-delta-small-r}}
%     \label{fig:small-r-privacy-amplification}
%     % Optional: Adjust vertical space below the caption if needed
%     \vspace{-10pt} 
% \end{wrapfigure}
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{fig/eps_vs_sigma_r10_r50.png}
    \caption{Privacy loss $\varepsilon$ v.s. noise scale $\sigma$ for $\delta = 1e-5$ and $d = 2000$: We compare our bound~(\Cref{thm:matrix-dp-proj-mechanism-small-r}), minimized over $\alpha$ with the Classical Gaussian mechanism~(\Cref{equ:gauss-delta-small-r}).}
    \label{fig:small-r-privacy-amplification}
    \vspace{-5mm}
\end{figure}
On \(\mathcal{G}_\alpha\), the effective squared sensitivity drops from \(\|\Delta V\|_F^2\) to \(\alpha\|\Delta V\|_F^2\), so the Gaussian term improves as \(\alpha\) decreases. Meanwhile \(\Pr(\mathcal{G}_\alpha^c)\) decreases as \(\alpha\) increases. Thus \(\alpha\) trades off a tighter Gaussian term against a rarer good event. This trade-off translates into a concrete improvement once we optimize over \(\alpha\) via simple numerical methods. As shown in \Cref{fig:small-r-privacy-amplification}, the resulting bound can strictly beat the Gaussian baseline in the small-\(r\) regime (with larger gains for smaller \(r\)). Intuitively, a random rank-\(r\) subspace captures only \(\approx r/d\) of the energy of a fixed direction. In the small-\(r\) regime, choosing \(\alpha\) just above this typical level keeps the failure probability small while still substantially tightening the Gaussian term. \Cref{cor:small-r-delta-improvement} in the Appendix makes this precise: if \(r\ll d\) and \(\log s \lesssim r\), an appropriate \(\alpha\) always outperforms the Gaussian baseline.


% Figure~\ref{fig:small-r-privacy-amplification} shows that optimizing our bound over \(\alpha\) can strictly outperform the Gaussian baseline in the small-\(r\) regime (with larger gains for smaller \(r\)).

% \begin{figure}
%     \centering
%     \includegraphics[width=0.6\linewidth]{fig/eps_vs_sigma_r10_r50.png}
%     \caption{Privacy loss $\varepsilon$ v.s. noise scale $\sigma$ for $\delta = 1e-5$ and $d = 2000$: We compare our bound~(\Cref{thm:matrix-dp-proj-mechanism-small-r}), minimized over $\alpha$ with the Classical Gaussian mechanism~(\Cref{equ:gauss-delta-small-r}).}
%     \label{fig:small-r-privacy-amplification}
% \end{figure}

To relate these bounds to common training procedures, note that the Gaussian baseline above is exactly the privacy accounting for standard DP-SGD. Recalling that by our notation \(V=\nabla_W \cL(W_t)^\top\), privatizing \(V\) directly (without conditioning on \(M\)) amounts to adding Gaussian noise to the full gradient, i.e., updating without any low-rank projection. We use \(\cA_2\) as a proxy for DP-LoRA-FA, but emphasize that it is not identical to the standard implementation: we add Gaussian noise to \(V^\top=\nabla_W \cL(W_t)\) and then apply the random projection, whereas DP-LoRA-FA adds noise after first multiplying by \(A^\top\). We focus on the former variant because it admits a more tractable theoretical analysis. Nonetheless, Appendix~\ref{app:subsec-comparison-dp-lora-small-r} shows that when analysing one training step, the two procedures inject noise of the same order, with high probability. For completeness, we include the standard DP-LoRA-FA implementation in our experiments.

For an empirical comparison, we fine-tune the linear head of a pretrained ResNet-50 on CIFAR-10 and evaluate our method (\ref{eq:M2} with privacy accounting from \Cref{thm:matrix-dp-proj-mechanism-small-r}) against DP-LoRA-FA and DP-SGD under the same privacy budget. Appendix~\ref{app:subsec-comparison-exp-details} provides implementation details (backbone, hyper-parameter grid, and accounting). 

\Cref{fig:comparison} (right) plots test accuracy versus the privacy budget $\varepsilon$ for $\delta = 10^{-4}$. In the small-\(\varepsilon\) regime, our method outperforms DP-SGD because the low-rank projection reduces the noise required to attain a fixed privacy level. DP-LoRA-FA shows the same effect, but only at even smaller \(\varepsilon\). As $\varepsilon$ grows, less noise is required noise for all methods and this noise advantage fades. For large $\varepsilon$ the accuracy gains from reduced noise are outweighed by the optimization bias introduced by the low-rank constraint, so DP-SGD matches or slightly outperforms our approach. 
In~\Cref{fig:comparison} (left), we isolate the effect of the low-rank projection by comparing our method with standard DP-LoRA-FA for varying ranks $r$, at fixed privacy budget ($\varepsilon \in \{0.2, 0.4\}$)\footnote{See results for more $\varepsilon$ in~\Cref{fig:best-acc-vs-r-more-eps}. }. While the two approaches are similar and, with high probability, add effective noise of the same order (see Appendix~\ref{app:subsec-comparison-dp-lora-small-r}), we observe that our Wishart projection consistently performs better, particularly at smaller ranks. This suggests that utility is influenced not only by the noise level, but also by the geometry of the random projection (applied to both the gradient matrix and the noise). Understanding when and why different projection distributions yield better utility is an interesting direction for future work. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/dp_lora_vs_ours_plots.pdf}
    \caption{Comparison of DP-SGD, DP-LoRA-FA, and our mechanism~(\ref{eq:M2}) using the privacy accounting of \Cref{thm:matrix-dp-proj-mechanism-small-r}.}
    \label{fig:comparison}
    \vspace{-7mm}
\end{figure}


==> icml2026/content/prelim.tex <==
We first review DP preliminaries, then introduce LoRA and show how it instantiates the projection mechanism.

Differential privacy limits how much the output distribution can change when a single data point is modified.
We say datasets $S, S'$ are neighbors, denoted $S \sim_H S'$, if they differ in a single entry (i.e., Hamming distance $d_H(S, S') = 1$).

% \begin{defn}[Neighboring datasets]
% Let $S,S'$ be datasets  of same size. We write $S \sim_H S'$ if they differ in exactly one entry, i.e.\ $d_H(S,S')=1$, where $d_H$ is the Hamming distance.
% \end{defn}

\begin{defn}[Differential privacy]\label{defn:dp}
A randomised algorithm $\cA: \cS \to \cY$ is $(\varepsilon,\delta)$-DP if for all measurable $E\subseteq\cY$ and all $S\sim_H S'$,
\[
\Pr(\cA(S)\in E)\le e^\epsilon\Pr(\cA(S')\in E)+\delta,
\]
with probability taken over the internal randomness of $\cA$.
\end{defn}
Differential privacy is commonly enforced by additive perturbations: adding noise to the output of a non-private query \(f\), calibrated to its $\ell_2$ sensitivity, 
\[
\Delta \coloneqq \max_{S\sim_H S'} \norm{f(S)-f(S')}_2.
\]
A canonical example is the Gaussian mechanism: 
\begin{lem}[Gaussian Mechanism]
\label{lem:gaussian-mech}
Let $f: \mathcal{S} \to \mathbb{R}^d$ be a function with $\ell_2$-sensitivity $\Delta$. For any $\epsilon, \delta \in (0, 1)$, the Gaussian mechanism $\mathcal{A}(S) = f(S) + Z$ is $(\epsilon, \delta)$-DP, for \[Z \sim \mathcal{N}(0, \sigma^2 I_d), \text{ where }
\sigma \ge \frac{2\Delta \sqrt{ \log(1.25/\delta)}}{\epsilon}.\]
\end{lem}


% \begin{lem}[Gaussian mechanism]\label{lem:gaussian-mech}
% Let $f:\cS\to\reals^d$ have sensitivity $\Delta$. The following mechanism is $(\epsilon,\delta)$-DP.
% \[
% \cA(S)=f(S)+Z,\qquad Z\sim \cN\br{0,\frac{2\Delta^2\log\frac{2}{\delta}}{\epsilon^2}I_d}
% \]
% \end{lem}

Restricting $\cA$ to datasets in $\cD \subseteq \cS$ gives DP guarantees \emph{conditioned on $\cD$}. This often reduces $\Delta$ and improves utility, but offers no privacy outside $\cD$. One way to obtain full privacy is to privately check whether the dataset belongs to $\cD$, e.g., via Propose-Test-Release~\cite{dwork2009differential}.


% Restricting the domain of $\cA$ to a dataset collection $\cD\subseteq \cS$ yields a DP guarantee \emph{conditioned on $\cD$}. In practice, this often reduces $\Delta$ and improvs utility but comes at the cost of not providing privacy on datasets outside the collection. Several approaches have been proposed in the literature to check whether a dataset indeed belongs to a collection \(\cD\), including the Propose-Test-Release mechanism~(PTR)~\cite{dwork2009differential}. 

\paragraph{LoRA is a Projection Mechanism}
\label{subsec:lora-priv}


% Before proceeding to our formal theoretical results, we first motivate our results using an application. 
Low-Rank Adaptation (LoRA;~\citet{hu2022lora}) is one of the most popular parameter-efficient fine-tuning approaches for Large Language Models. It augments a pretrained weight matrix $W_0\in\reals^{n\times d}$ by a \emph{low-rank} update:
\[
W = W_0 + BA, \; B\in\R^{n\times r}, \;A\in\reals^{r\times d}, \; r\ll\min\bc{d,n}.
\]
By freezing $W_0$ and only optimizing the smaller matrices $(B, A)$, LoRA reduces computational cost while preserving the base model's capabilities. 

LoRA-FA\citep{lorafa2023} is a variant that fixes $A$ and only updates $B$. When $A$ is initialized Gaussian and then \emph{frozen}, we update $B$ by
\[
B_{t+1}\;=\;B_t - \eta\,(\nabla_W \cL(W_t))A^\top.
\]
Then after $T$ steps, we can write
\begin{equation}\label{eq:weight-final}
W_T \;=\; W_0 - \eta \sum_{t=1}^T \big(\nabla_W \cL(W_t)\big)\,(A^\top A).
\end{equation}
Thus each step uses a gradient \(\nabla_W \cL(W_t) \in \R^{n \times d}\) that is \emph{right-projected} by the random matrix $A^\top A$ (a rank-$r$ Wishart). Right multiplying a vector or matrix by a randomly sampled Wishart is precisely the projection mechanism studied in this work. Prior work~\citep{malekmohammadi2025lowrankadaptationsecretlyimitates} suggested that this random projection structure may yield DP guarantees. However, as we show in \Cref{sec:proj-mechanism-vector}, the matrix-valued projection mechanism is not DP in general (see \Cref{prop:neg-res}). 



However, our results in~\Cref{sec:proj-mechanism-matrix} show that noisy versions of the projection mechanism enjoy $(\varepsilon, \delta)$-DP guarantees that in certain regimes are stronger than simple noise addition (i.e., Gaussian mechanism) would suggest due to the randomness stemming from the projection.


% we believe that the fact that the very popular algorithm already enjoys these guarantees, as has been hinted by previous work~\citep{malekmohammadi2025lowrankadaptationsecretlyimitates} is already interesting. Additionally, in~\Cref{sec:proj-mechanism-matrix} we also discuss algorithmic techniques to amplify these privacy guarantees.

==> icml2026/content/vecproj.tex <==
We study the privacy properties of the projection mechanism~(\Cref{defn:projection-mech}). We first analyze the special case of vector-valued queries \(f:\cS\to\reals^d\) and show in Section~\ref{subsec:privacy-guarantee-vector} that it is differentially private under an alignment assumption. In contrast, for matrix-valued queries we prove a negative result: \Cref{prop:neg-res} shows the privacy loss is unbounded (\(\epsilon=\infty\) for any \(\delta<1\)). This also implies that LoRA-FA and LoRA is not private. 

\subsection{Privacy Guarantees for Vector-Valued Functions}\label{subsec:privacy-guarantee-vector}
Let \(f:\cX^n\to\reals^d\) be a query with \(\|f(S)\|_2=1\) for all \(S\); this normalization can always be enforced by scaling, and we assume it throughout. For a dataset collection \(\cD\subset\cX^n\), define the \emph{minimum alignment}
\begin{equation}
\label{eq:min-alignment-vec}
\rho(\cD,f)\coloneqq \min_{\substack{S,S'\in\cD\\ S\sim_H S'}} f(S)^\top f(S') \in [-1,1].
\end{equation}
When the context is clear, we write \(\rhoalign:=\rho(\cD,f)\). Large $\rhoalign$ means that neighbouring query outputs are nearly co-directional. In this regime the laws of $Mf(S)$ and $Mf(S')$ are harder to distinguish, leading to tighter $(\varepsilon_\rho,\delta_\rho)$ guarantees~(\Cref{fig:vector-case-simulation}). Crucially, much like a sensitivity parameter in additive mechanisms, $\rhoalign$ is a property fixed by the dataset collection \(\cD\) and the query $f$ and is not controlled by the projection mechanism itself. One can also preprocess the data to improve the alignment $\rho$ through e.g. noise addition. See Appendix~\ref{app:vecprivamplification-and-applications} for details. 

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{llccccc}
\toprule
\multirow{2}{*}{\textbf{Setting}} & \multirow{2}{*}{\textbf{Metric}} &
\multicolumn{5}{c}{\textbf{Rank $r$}} \\
\cmidrule(lr){3-7}
 & & \textbf{16} & \textbf{32}  & \textbf{128} & \textbf{256} & \textbf{512} \\
\midrule
\multirow{2}{*}{Train from scratch} 
& Test Acc (\%) & 57.31 & 61.76     & 66.36 & 67.34 & 68.36 \\
& AUC (\%)      & 99.86 & 99.64     & 100.00 & 100.00 & 100.00 \\
\midrule
\multirow{2}{*}{Pretrain+Finetune } 
& Test Acc (\%) & 75.98 & 75.63  & 76.12 & 76.04 & 76.45 \\
& AUC (\%)      & 99.81 & 99.98  & 100.00 & 100.00 & 100.00 \\
\bottomrule
\end{tabular}
\vspace{1mm}
\caption{Membership inference attack performance for noise-free LoRA under a static-poison canary construction.}
\label{tab:mia-noiseless}
\vspace{-5mm}
\end{table*}

% To recall, for a given \(r,\sigma\), the projection mechanism samples a Wishart matrix
% \begin{equation*}
%     \begin{aligned}
%         M \coloneqq \sum_{i=1}^r z_i z_i^\top = ZZ^\top,&~Z=\bs{z_1,\cdots,~ z_r}\in\reals^{d\times r} \\
%         \text{where}\quad
%   z_i&~\stackrel{\text{i.i.d.}}{\sim}\cN\br{0,\sigma^2 I_d},
%     \end{aligned}
% \end{equation*}
% \[
%   M \coloneqq \sum_{i=1}^r z_i z_i^\top = ZZ^\top,\qquad~\text{where}~\quad
%   z_i\stackrel{\text{i.i.d.}}{\sim}\cN\br{0,\sigma^2 I_d},\ Z=\bs{z_1,\cdots,~ z_r}\in\reals^{d\times r},
% \]
%and releases $Mf(S)$. 

% Let $f:\cX^n\to\reals^d$ satisfy $\norm{f(S)}_2=1$ for all $S$ (this normalization can be enforced by scaling). For a dataset collection $\cD\subset\cX^n$  and query function \(f\) define their \emph{minimum alignment} 
% \begin{equation}
%     \label{eq:min-alignment-vec}
% \rho\br{\cD,f} \coloneqq \min_{S\sim_H S',S,S'\in\cD} f\br{S}^\top f\br{S^\prime}\in\bs{-1,1}.
% \end{equation}
% For purposes of brevity, we will misuse notation slightly and write \(\rhoalign\coloneqq \rho(\cD, f)\), when the context is clear. Large \(\rhoalign\) indicates that outputs of neighbouring datasets are co-directional, thus the images \(Mf\br{S}\) and \(Mf\br{S^\prime}\) overlap substantially yielding meaningful~\(\br{\epsilon_\rho,\delta_\rho}\)-DP guarantees. Importantly, the \(\rhoalign\) parameter is determined by the dataset collection and the query function, akin to sensitivity in additive DP mechanisms, and does not depend on algorithmic choices made in the projection mechanism. However, just like clipping, we discuss algorithmic techniques to amplify the privacy guarantees in~\Cref{sec:privacy-amplification}. Unlike \(\rhoalign\), the projection mechanism chooses $r$, the degrees of freedom of the Wishart distribution. As $r$ increases, we sample additional columns of $Z$, producing a higher-rank Wishart matrix $M=ZZ^\top$. 
% We see that larger $r$ leads to smaller $\varepsilon$ and $\delta$, this intuitively follows as larger $r$ requires more random bits in the sampling. Smaller $r$ can still be attractive in practice, as it reduces memory and compute. Thus selecting $r$ entails a \emph{trade-off between efficiency (smaller $r$) and tighter privacy guarantees (larger $r$)}.


% We use the alignment parameter $\rho$ in the vector case to quantify how much privacy the random projection can provide.  For large $\rho$, the images $Mf(S)$ and $Mf(S')$ overlap substantially, yielding meaningful $(\varepsilon_\rho,\delta_\rho)$ guarantees. The alignment $\rho$ is determined by the data $\mathcal{D}$ and the query function $f$, therefore the mechanism cannot change it (however we do discuss amplification strategies in~\Cref{sec:privacy-amplification}). By contrast, the projection mechanism \emph{does} let us choose $r$ the degrees of freedom of the Wishart draw. As $r$ grows, we sample additional columns of $Z$, producing a higher-rank Wishart matrix $M=ZZ^\top$. We also see that larger $r$ leads to smaller $\varepsilon$ and $\delta$, this intuitively follows as larger $r$ leads to more randomness. Smaller $r$ can still be attractive in practice, as it reduces memory and compute. Thus selecting $r$ entails a \emph{trade-off between efficiency (smaller $r$) and tighter privacy guarantees (larger $r$)}.ld be non-positive).


% \begin{restatable}{thm}{VecPrivacy}
%     \label{thm:privacy-lora-vector-version}
%     For a dataset collection $\cD$ and a query function $f$ with outputs in $\bR^d$, let $\rho > 0$ be the minimum alignment for $f, \cD$ as defined in~\Cref{eq:min-alignment-vec}. Then, for any $R>(\sqrt{d} + \sqrt{r})^2$, $0 < t < \frac{1}{2}\abs{\rho\sigma^2\br{\sqrt{r}-\sqrt{d}}}$ (where for the $r < d$ we have no upper bound on $t$), and $\eta > 0$ the projection mechanism with rank $r $ and variance $\sigma^2$ is $(\varepsilon_\rho, \delta_\rho)$-DP on $\cD$, where
%     \[
%     \delta_\rho =
%     \begin{cases}
%       1 - \bar{\Phi}\!\left( \frac{ t (1 - \rho)  - \rho \eta}{\sqrt{(1 - \rho^2)(t + \eta)}}\right)
%       \bP(\chi_r^2 > t + \eta) + 2\exp\!\bigl(-c(\sqrt{R} - \sqrt{d} - \sqrt{r})^2\bigr),
%       & r < d,\\[4pt]
%       4e^{-(\sqrt{r}-\sqrt{d})^2/8} + 2e^{-c(\sqrt{d}+\sqrt{r})^2},
%       & r \ge d.
%     \end{cases}
%     \]
%     \[\varepsilon_\rho \leq \frac{\abs{d-r - 1}}{2}\log \left( \rho + \sqrt{1 - \rho^2} \sqrt{\frac{R^2}{t^2} - 1} \right) + \frac{R^3 \sqrt{2(1-\rho)}}{2 t^2}\]
% \end{restatable}

Let \(t_{\ell}(\cdot)\) and \(\kappa_{\ell}(\cdot)\) denote the quantile functions of the Student-\(t\) and \(\chi^2\) distributions, respectively, each with \(\ell\) degrees of freedom.
    
\begin{restatable}{thm}{vecprivacynew}\label{thm:vec-alt}
    For a dataset collection $\cD$ and a query function $f$ with outputs in $\bR^d$, let $\rho > 0$ be the minimum alignment for $f$ on $\cD$ as defined in~\Cref{eq:min-alignment-vec}. Let $\delta' > 0$. If $\rho > \frac{t_r(1-\delta')}{\sqrt{r + t_r(1-\delta')^2}}$, then, the projection mechanism~(\Cref{defn:projection-mech}) with rank $r$ is $(\varepsilon_\rho, \delta_\rho)$-DP on $\cD$, with
    \[
    \begin{aligned}
    \delta_\rho &=
      \bE_{x\sim \cX_r^2} \bs{\Phi\br{-\frac{\rho \sqrt{x}}{\sqrt{1-\rho^2}}}} + 3\delta'
    \end{aligned}
    \]
    \[
    \begin{aligned}
     \varepsilon_\rho  \leq \frac{d - r + 1}{2} \ln \br{\rho + K} + \frac{(1-\rho + K)\kappa_{d + r -1}(1-\delta')}{2(\rho - K)}
    \end{aligned}
    \]
    where $K = \sqrt{\frac{1-\rho^2}{r}}t_r(1-\delta')$.
\end{restatable}

% \yh{We can further write $\bE_{x\sim \cX_r^2} \bs{\Phi\br{-\frac{\rho \sqrt{x}}{\sqrt{1-\rho^2}}}}  = 1-F_{t_r}\br{\frac{\rho\sqrt{r}}{\sqrt{1-\rho^2}}}$, where $F_{t_r}$ denote the CDF of student t distribution with degree of freedom r. }

% \begin{wrapfigure}{r}{0.5\linewidth}
%     \centering\vspace{-15pt}\includegraphics[width=\linewidth]{fig/epsilon_vs_r_fixed_d.png}
%     \caption{Privacy loss $\varepsilon$ v.s. rank $r$ at $\delta = 0.01$ and $d = 400$: Monte Carlo simulation of exact privacy profile in~\Cref{thm:vec-alt}.}
%     \label{fig:vector-case-simulation}
%     % Optional: Adjust vertical space below the caption if needed
%     \vspace{-10pt} 
% \end{wrapfigure}
% \begin{figure}
%     \vspace{-5pt}
%     \centering
%     \includegraphics[width=0.5\linewidth]{fig/epsilon_vs_r_fixed_d.png}
%     \caption{Privacy loss $\varepsilon$ v.s. rank $r$ at $\delta = 0.01$ and $d = 400$: Monte Carlo simulation of exact privacy profile and~\Cref{thm:vec-alt}.}
%     \label{fig:vector-case-simulation}
%     \vspace{-20pt} 
% \end{figure}
\begin{figure}
    \vspace{-5pt}
    \centering
    \includegraphics[width=0.55\linewidth]{fig/epsilon_vs_r_fixed_d.png}
    \caption{Privacy loss $\varepsilon$ v.s. rank $r$ at $\delta = 0.01$ and $d = 400$: Monte Carlo simulation of exact privacy profile and~\Cref{thm:vec-alt}.}
    \label{fig:vector-case-simulation}
    \vspace{-15pt} 
\end{figure}
Here $r$ is the rank of the Wishart matrix $M=ZZ^\top$ with $Z\in\mathbb{R}^{d\times r}$, and is an algorithmic choice.
As illustrated in~\Cref{fig:vector-case-simulation}, for fixed $\delta$ the resulting $\varepsilon$ depends non-monotonically on $r$. This reflects two competing effects: smaller $r$ makes $M$ lower-rank, confining the output to a lower-dimensional subspace and potentially reducing leakage via compression; but it also relies on fewer Gaussian directions, increasing tail risk and potentially weakening the \((\varepsilon,\delta)\) guarantee.

\noindent\textbf{On the dependence of $\rhoalign$ on $n$.}
The minimum alignment $\rhoalign$ measures how much the direction of the normalised query can change under a single record change. For average-type queries, one replacement perturbs the unnormalised vector by $O(1/n)$, which typically yields $\rhoalign = 1-\widetilde{O}(1/n^2)$. Concretely, let $\tilde f(S)=\frac{1}{n}\sum_{i=1}^n g(x_i)$ with $\|g(x)\|_2\le L$ and assume $\inf_{S\in\cD}\|\tilde f(S)\|_2\ge c_0>0$. Then for neighboring datasets $S, S'$, we have $\|\tilde f(S)-\tilde f(S')\|_2\le 2L/n$. Defining $f(S)\coloneqq \tilde f(S)/\|\tilde f(S)\|_2$ gives $\|f(S)-f(S')\|_2\le 4L/(c_0 n)$ and hence $\rhoalign \ge 1-\frac{8L^2}{c_0^2 n^2}$, using $1-u^\top v=\tfrac12\|u-v\|_2^2$ for unit vectors.
The same argument applies to mini-batch gradients: for $\tilde f(B)=\frac{1}{|B|}\sum_{x\in B}\nabla \ell(\theta;x)$, if $\|_2\nabla \ell(\theta;x)\|_2\le L$ and $\|\tilde f(B)\|_2$ is bounded away from zero, then $\rhoalign = 1-\widetilde{O}(1/|B|^2)$.

\subsection{Negative Results for Matrix-Valued Functions}\label{subsec:matrix-negative-result}

\Cref{thm:vec-alt} establishes \((\varepsilon,\delta)\)-DP for the projection mechanism on \emph{vector}-valued queries under an alignment condition. Since the LoRA-FA update can be cast as the same mechanism with \emph{matrix}-valued outputs (see~\Cref{sec:prelim}), one might expect an analogous guarantee for matrices and thus privacy for LoRA-FA. We show this is false: without additive noise, the matrix-valued projection mechanism is not DP.

\begin{proposition}\label{prop:neg-res}
    Let $f:\cS\to \bR^{n\times d}$ be a non-trivial function and $\cA(S)$ be the projection mechanism~(\Cref{defn:projection-mech}) with query function $f$. Then, there exists two neighboring datasets $S, S' \in \cS$ and a measurable event $E$ with 
    \[
    \begin{aligned}
        \Pr(\cA(S)\in E) = 1,\quad
        \Pr(\cA(S')\in E)= 0
    \end{aligned}
    \]
    Consequently, $\cA$ is not $(\varepsilon, \delta)$-DP for any $\varepsilon$ and any $\delta <1$.
\end{proposition}
\noindent\textbf{Proof intuition: }
Let \(V:=f(S)\) and \(V':=f(S')\). As $V\neq V'$ such that $V - V'\neq 0$ and $\text{rank}(V - V') = s \geq 1$. Given $S$ the mechanism outputs the random variable \(Y=VM =  VZ Z^\top\), where each column $z_i$ of $Z$ is i.i.d. $\cN(0, I_d/r)$. For the two outputs to coincide we require $(V - V') M = 0$, i.e. $ (V - V') Z= 0$: every random direction $z_i$ must be orthogonal to the rowspace of $(V - V') $. As $\text{rank}(V - V') = s$, its orthogonal complement is a $(d - s)$-dim subspace. A continuous Gaussian vector $z_i$ lands in a fixed lower dimensional subspace with probability 0. Hence, $VM \neq V'M$ almost surely. Taking $E = \text{Supp}(VM)$ concludes the proof. (See~\Cref{lem:image-overlap-measure-zero}).

\Cref{prop:neg-res} extends beyond our abstract projection mechanism to directly rule out “privacy for free” arising from LoRA’s random initialization. Specifically, the first update step of standard LoRA (where $B_0 = 0$) is equivalent to the~\Cref{defn:projection-mech}, implying standard LoRA cannot satisfy DP without additional additive noise (See Appendix~\ref{app:negative-result-lora} for detailed explanation).

Motivated by the negative result above, we test noise-free LoRA against a membership inference attack (MIA). We run 2000 independent trials on CIFAR-10 using the popular static-poison canary construction~\cite{nasr2021adversary} in two regimes: (i) training from scratch, and (ii) pretraining followed by fine-tuning on CIFAR-10. \Cref{tab:mia-noiseless} reports test accuracy and ROC-AUC. Across both regimes and all ranks, the attack achieves near-perfect separability (AUC $\approx 1$), consistent with the non-overlap intuition suggested by the theory. See Appendix~\ref{app:exp-mia} for details. 

These findings do not conflict with prior work showing that LoRA can reduce MIA success~\citep{malekmohammadi2025lowrankadaptationsecretlyimitates,hong2025evaluating}, since MIA performance depends strongly on the threat model. We consider a strong adversary who knows all but one training records and can choose an adversarial canary, mirroring DP’s worst-case auxiliary-information setting where the guarantee must hold for any choice of differing example. Our work shows that under a classical DP style adversary, LoRA is not private. 


==> icml2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

